Variation across Scales: Measurement Fidelity under Twitter Data Sampling

A comprehensive understanding of data quality is the cornerstone of measurement studies in social media research. This paper presents in-depth measurements on the effects of Twitter data sampling across different timescales and different subjects (entities, networks, and cascades). By constructing complete tweet streams, we show that Twitter rate limit message is an accurate indicator for the volume of missing tweets. Sampling also differs significantly across timescales. While the hourly sampling rate is influenced by the diurnal rhythm in different time zones, the millisecond level sampling is heavily affected by the implementation choices. For Twitter entities such as users, we find the Bernoulli process with a uniform rate approximates the empirical distributions well. It also allows us to estimate the true ranking with the observed sample data. For networks on Twitter, their structures are altered significantly and some components are more likely to be preserved. For retweet cascades, we observe changes in distributions of tweet inter-arrival time and user influence, which will affect models that rely on these features. This work calls attention to noises and potential biases in social data, and provides a few tools to measure Twitter sampling effects.

==> Measuring Sampling Effects in Twitter Streaming API/abstract.tex <==
%!TEX root = TwitterSampling.tex

\begin{abstract}
A comprehensive understanding of data quality is the cornerstone of measurement studies in social media research.
This paper presents in-depth measurements on the effects of Twitter data sampling across different timescales and different subjects (entities, networks, and cascades).
By constructing complete tweet streams, we show that Twitter rate limit message is an accurate indicator for the volume of missing tweets.
Sampling also differs significantly across timescales.
While the hourly sampling rate is influenced by the diurnal rhythm in different time zones, the millisecond level sampling is heavily affected by the implementation choices.
For Twitter entities such as users, we find the Bernoulli process with a uniform rate approximates the empirical distributions well.
It also allows us to estimate the true ranking with the observed sample data.
For networks on Twitter, their structures are altered significantly and some components are more likely to be preserved.
For retweet cascades, we observe changes in distributions of tweet inter-arrival time and user influence, which will affect models that rely on these features.
This work calls attention to noises and potential biases in social data, and provides a few tools to measure Twitter sampling effects.
\end{abstract}

% A comprehensive understanding of data quality is the cornerstone of measurement studies in social media research. This paper presents in-depth measurements on the effects of Twitter data sampling across different timescales and different subjects (entities, networks, and cascades). By constructing complete tweet streams, we show that Twitter rate limit message is an accurate indicator for the volume of missing tweets. Sampling also differs significantly across timescales. While the hourly sampling rate is influenced by the diurnal rhythm in different time zones, the millisecond level sampling is heavily affected by the implementation choices. For Twitter entities such as users, we find the Bernoulli process with a uniform rate approximates the empirical distributions well. It also allows us to estimate the true ranking with the observed sample data. For networks on Twitter, their structures are altered significantly and some components are more likely to be preserved. For retweet cascades, we observe changes in distributions of tweet inter-arrival time and user influence, which will affect models that rely on these features. This work calls attention to noises and potential biases in social data, and provides a few tools to measure Twitter sampling effects.


==> Measuring Sampling Effects in Twitter Streaming API/images/fig-bipartite-clusters.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{figure}[tbp]
    \centering
    \includegraphics[width=.99\columnwidth]{image-files/measure_bipartite_cluster_flow.pdf}
	\caption{The change of clusters from complete set to sample set.
	Each cell denotes the volume (top number) and the ratio (bottom percentage) of entities (users and hashtags) that traverse from a complete cluster to a sample cluster.
	Clusters are ordered to achieve maximal ratios along the diagonal.}
	\label{fig:bipartite-cluster}
\end{figure}

==> Measuring Sampling Effects in Twitter Streaming API/images/fig-bipartite-robust.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.474\textwidth]{image-files/metrics_kendall.pdf}
	\caption{Kendall's $\tau$ for different network metrics. \textbf{(a)} user; \textbf{(b)} hashtag.}
	\label{fig:bipartite-robust}
\end{figure}

==> Measuring Sampling Effects in Twitter Streaming API/images/fig-bowtie-stats.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{figure}[tbp]
    \centering
    \includegraphics[width=.99\columnwidth]{image-files/measure_bowtie_flow.pdf}
	\caption{The change of bow-tie components from complete set to sample set.
	Each cell denotes the volume (top) and the ratio (bottom) of users that traverse from a component in complete set to a component in sample set.}
	\label{fig:measure-bowtie-stats}
\end{figure}

==> Measuring Sampling Effects in Twitter Streaming API/images/fig-bowtie.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.8\columnwidth]{image-files/bow_tie.pdf} 
	\caption{Visualization of bow-tie structure in complete set. The black number indicates the relative size of component in the complete set, \textcolor{blue}{blue} number indicates the relative size in the sample set.
% 	Black text denotes the number and ratio of users in each component.
% 	Blue text denotes the number and ratio of retweets between two components.
% 	For example, users in the IN component retweet the content emitted by users in the LSCC component 39.9 million times, which accounts for 48.5\% retweets in our dataset.
    }
	\label{fig:measure-bowtie}
\end{figure}

==> Measuring Sampling Effects in Twitter Streaming API/images/fig-cascade.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{figure}[tbp]
    \centering
    \includegraphics[width=.99\columnwidth]{image-files/cascades_measures.pdf}
	\caption{CCDFs of \textbf{(a)} inter-arrival time and \textbf{(b)} relative potential reach.}
	\label{fig:measure-cascade}
\end{figure}

==> Measuring Sampling Effects in Twitter Streaming API/images/fig-entity-binomial.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{figure}[tbp]
    \centering
    \includegraphics[width=.99\columnwidth]{image-files/entity_binomial.pdf}
	\caption{\textbf{(a)} D-statistic between empirical distribution and binomial distribution for the number of tweets a user posts.
 	\textbf{(b)} The probability distribution of observing $n_s$ times in the sample set when $n_c{=}20$.}
	\label{fig:measure-entity-binomial}
\end{figure}

==> Measuring Sampling Effects in Twitter Streaming API/images/fig-entity-frequency.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{figure}[tbp]
    \centering
    \includegraphics[width=.99\columnwidth]{image-files/entity_freq_dist.pdf}
	\caption{The frequency distributions of \textbf{(a)} user posting and \textbf{(b)} hashtag. The x-axis starts at 0 rather than 1, as the sample set and uniform random sample both have missing entities.}
	\label{fig:entity-frequency}
\end{figure}


==> Measuring Sampling Effects in Twitter Streaming API/images/fig-entity-negbin.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{figure}[tbp]
    \centering
    \includegraphics[width=.99\columnwidth]{image-files/entity_negative_binomial.pdf}
	\caption{\textbf{(a)} D-statistic between empirical distribution and negative binomial distribution for the number of tweets a user posts.
	\textbf{(b)} The probability distribution of posting $n_c$ times in the complete set when $n_s{=}13$.}
    \label{fig:entity-negbin}
\end{figure}

==> Measuring Sampling Effects in Twitter Streaming API/images/fig-lang-vol.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{figure}[tbp]
    \centering
    \includegraphics[width=.99\columnwidth]{image-files/tweet_lang_vol.pdf} \\ 
	\caption {Hourly tweet volumes in \yt dataset. \textbf{(a)} Japanese+Korean; \textbf{(b)} other languages.
	black line: temporal mean tweet volumes; color shades: 95\% confidence interval.}
	\label{fig:tweet-lang-vol}
\end{figure}

==> Measuring Sampling Effects in Twitter Streaming API/images/fig-relative-importance.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.47\textwidth]{image-files/relative_importance.pdf}
	\caption{Changes of relative importance from the complete set to the sample set. \textbf{(a)} user; \textbf{(b)} hashtag.}
	\label{fig:relative_importance}
\end{figure}

==> Measuring Sampling Effects in Twitter Streaming API/images/fig-sampling-rate.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{figure}[tbp]
    \centering
    \includegraphics[width=.99\columnwidth]{image-files/temporal_sampling_rates.pdf} \\
	\caption{Sampling rates are uneven \textbf{(a)} in different hours or \textbf{(b)} in different milliseconds.
	black line: temporal mean sampling rates; color shades: 95\% confidence interval.}
	\label{fig:temporal-sampling-rates}
\end{figure}

==> Measuring Sampling Effects in Twitter Streaming API/images/fig-top-rank.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{figure}[tbp]
    \centering
    \includegraphics[width=.99\columnwidth]{image-files/entity_rank.pdf}
	\caption{\textbf{(a)} Observed ranks in the sample set (x-axis) vs. true ranks in the complete set (y-axis).
	\textbf{(b)} Estimated ranks improve the agreement with the ground-truth ranks.
	\textbf{(c)} user \textit{WeltRadio}, observed/true/estimated ranks: 15/50/50.
	\textbf{(d)} user \textit{bensonbersk}, observed/true/estimated ranks: 66/42/52.
	\textcolor{blue}{blue}/\textcolor{red}{red} shades: sample tweet volume; grey shades: complete tweet volume; black line: estimated tweet volume.}
	\label{fig:top-rank}
\end{figure}

==> Measuring Sampling Effects in Twitter Streaming API/images/fig-validate-ratemsg.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{figure*}[tbp]
    \centering
	\includegraphics[width=2.09\columnwidth]{image-files/validate_ratemsg.pdf}
	\caption{\textbf{(a)} Collected and missing tweets in an 11-second interval. \textcolor{blue}{blue} circle: collected tweet; black cross: missing tweet; black vertical line: rate limit message. \textcolor{ForestGreen}{green} number: estimated missing volume from rate limit messages; black number: count of missing tweets compared to the complete set.
	\textbf{(b)} MAPE of estimating the missing volumes in the rate limit segments.}
	\label{fig:data-validate-ratemsg}
\end{figure*}


==> Measuring Sampling Effects in Twitter Streaming API/sec-background.tex <==
%!TEX root = TwitterSampling.tex

% ====================================================
\section{Related work}
\label{sec:related}
% ====================================================

% ====================================================
\header{Studies on Twitter APIs.}
Twitter has different levels of access (Firehose, Gardenhose, Spritzer) and different ways to access (search API, sampled stream, filtered stream). 
As the complete data service (Firehose) incurs excessive costs and requires severe storage loads, we only discuss the free APIs.

\begin{itemize}[leftmargin=*]
  \item Twitter search API returns relevant tweets for a given query, but it only fetches results published in the past 7 days~\cite{twittersearch}.
  The search API also bears the issue of data attrition.
  Research using this API to construct a ``complete'' dataset would inevitably miss parts of desired tweets~\cite{wang2015should} since tweet creation and deletion are highly dynamic~\cite{almuhimedi2013tweets}.
  To overcome this limitation, researchers can pivot to the streaming APIs.
  
  \item Twitter sampled streaming API returns roughly 1\% of all public tweets in realtime~\cite{twittersample}.
  \citet{pfeffer2018tampering} detailed its sampling mechanism and identified potential tampering behaviors.
  % \citet{ghosh2013sampling} compared the 1\% sampling and expert sampling.
  % They observed that elite users share more trustworthy content and react faster to breaking events.
  \citet{gonzalez2014assessing} examined the biases in the retweet network from the 1\% sample and the search API.
  While the 1\% sample may be treated as a representative sample of overall Twitter activities~\cite{morstatter2014biased,kergl2014endogenesis}, data filtering can only be conducted post data collection.
  Therefore, it is not suitable to create ad hoc datasets, e.g., tracking \textit{all} tweets that contain the hashtag \texttt{\#metoo}.
  
  \item Twitter filtered streaming API collects tweets matching a set of prescribed predicates in realtime~\cite{twitterfilter}.
  Suppose that the streaming rate is below Twitter limit, the pre-filtering makes the filtered stream possible to construct the complete datasets without using the costly Firehose stream, e.g., on social movements~\cite{de2016social} and on news outlets~\cite{mishra2016feature}.
  We focus on the scenes where the data streams are sampled.
  The most relevant work is done by \citet{morstatter2013sample}, in which they compared the filtered stream to the Firehose, and measured the discrepancies in various metrics.
  We extend the scope of measured subjects.
  Furthermore, we take a step to correct the sampling effects on entity measures.
\end{itemize}

Twitter sampling is deterministic~\cite{joseph2014two}, therefore, simply stacking crawlers with the same predicates will not yield more data.
However, users can improve the sample coverage by splitting the keyword set into multiple disjoint predicate sets, and monitoring each set with a distinct subcrawler~\cite{sampson2015surpassing}.
% ====================================================

% ====================================================
\header{Effects of missing social data.}
% The fairness problem has received growing attention in academic studies.
Social data, which records ubiquitous human activities in digital form, plays a fundamental role in social media research.
% \citet{boyd2012critical} pointed out the necessity to interrogate the assumptions and biases in data.
% \citet{ruths2014social} discussed the biases and flaws in social media data.
Researchers have pointed out the necessity to interrogate the assumptions and biases in data~\cite{boyd2012critical,ruths2014social}.
\citet{tufekci2014big} outlined four issues on data representativeness and validity.
% including but not limited to under/over-representative and completely missing data.
The hidden data biases may alter some research conclusions and even impact human decision making~\cite{olteanu2019social}.

\citet{gaffney2018caveat} identified gaps where data is unevenly missing in a widely used Reddit corpus.
They suggested strong risks in research that concerns user history or network information, and moderate risks in research that uses aggregate counts.
In this work, we use these qualitative observations as starting points and present a set of in-depth quantitative measurements.
We corroborate the risks in user history study and network analysis.
And we show how the complete counting statistics can be estimated.
% ====================================================

% ====================================================
\header{Sampling from graphs and cascades.}
\citet{leskovec2006sampling} studied different graph sampling strategies for drawing representative samples.
\citet{wagner2017sampling} considered how sampling impacts the relative ranking of groups in the attributed graphs.
% Unlike \citet{morstatter2013sample}, we take account of the edge weights and self-loops in the retweet network.
The effects of graph sampling has been extensively discussed by \citet{kossinets2006effects}.
In this work, the missing tweets can cause edge weights to decrease, and some edges to even disappear.
On sampling a cascade, \citet{de2010does} found that combining network topology and contextual attributes distorts less the observed metrics.
\citet{sadikov2011correcting} proposed a \textit{k}-tree model to uncover some properties from the sampled data.
They both sampled the cascades via different techniques (e.g., random, forest fire) and varying ratios.
In contrast, the sampling in this work is an artifact of proprietary Twitter sampling mechanisms, and beyond the control of the users.
% ====================================================


==> Measuring Sampling Effects in Twitter Streaming API/sec-cascade.tex <==
%!TEX root = TwitterSampling.tex

% ====================================================
%\section{Measures of cascades}
\section{Impacts on retweet cascades}
\label{sec:cascade}

Information diffusion is perhaps the most studied social phenomenon on Twitter.
A retweet cascade consists of two parts: a root tweet and its subsequent retweets.
A number of models have been proposed for modeling and predicting retweet cascades~\cite{zhao2015seismic,mishra2016feature,martin2016exploring}.
However, these usually make the assumption of observing all the retweets in cascades.
In this section, we analyze the impacts of Twitter sampling on retweet cascades and identify risks for existing models.
We first construct cascades without missing tweets from the complete set.
Next, we measure the sampling effects for some commonly used features in modeling retweet cascades, e.g., inter-arrival time and potential reach.

\header{Constructing complete cascades.}
When using the filtered streaming API, if a root tweet is observed, the API should return all its retweets.
This is because the API also tracks the keywords in the \texttt{retweeted\_status} field of a tweet (i.e., the root tweet), which allows us to construct a set of complete cascades from the complete set.
In the sample set, both the root tweet and any of its retweets could be missing.
If the root tweet is missing, we miss the entire cascade.
If some retweets are missing, we observe a partial cascade.
\Cref{table:cascade} lists the obtained cascades in the complete and the sample sets.
Notably, there are 3M cascades in the complete set, but only 1.17M in the sample set (38.85\%), out of which only 508k (16.88\%) cascades are complete and their sizes are relatively small (i.e., they don't miss any retweet, max cascade size: 23, mean size: 1.37).
Prior literature~\cite{zhao2015seismic} often concentrates on retweet cascades with more than 50 retweets.
%Consistent with , we filter out cascades with less than 50 retweets.
There are 99,952 such cascades in the complete set, but only 29,577 in the sample set, out of which none is complete.

% \header{Do larger cascades miss more tweets?}

\header{Inter-arrival time.} One line of work models the information diffusion as point processes~\cite{zhao2015seismic,mishra2016feature}.
These models use a memory kernel as a function of the time gap $\Delta t$ between two consecutive events, which is also known as inter-arrival time.
\Cref{fig:measure-cascade}(a) plots the CCDFs of inter-arrival times in the complete and the sample sets.
The distribution shifts right, towards larger values.
This is expected as the missing tweets increase the time gap between two observed tweets.
The median inter-arrival time is 22.9 seconds in the complete set (black dashed line), meaning 50\% retweets happen within 23 seconds from last retweet.
After sampling, the median increases almost 5-fold to 105.7 seconds (\textcolor{blue}{blue} dashed line).
For research that uses tweet inter-arrival time, this presents the risk of miss-calibrating models and of underestimating the virality of the cascades.

\input{tables/tab-cascade.tex}

\input{images/fig-cascade.tex}

\header{Potential reach.}
%The capability to diffuse is related to the influence of current retweeters.
Online influence is another well-studied phenomenon on Twitter, and one of its proxies is the number of followers of a user.
We define potential reach as the total number of all observed retweeters' followers.
This approximates the size of the potential audience for the root tweet.
We compute the relative potential reach as the ratio of potential reach in the sample cascade against that in the complete cascade, and we plot the CCDFs in \Cref{fig:measure-cascade}(b).
%The maximal observation window is 14 days.
When observing cascades for as much as 14 days, 50\% of the cascades have the relative potential reach below 0.544.
This indicates that when using the sampled Twitter data, researchers can severely underestimate the size of the potential audience.
Another common setting is to perform early prediction, i.e., after observing 10 minutes or 1 hour of each retweet cascade.
%We thus plot the relative potential reach for the observation within the first 10 minutes and 1 hour after root tweet.
\Cref{fig:measure-cascade}(b) shows that the relative potential reach is more evenly distribution for shorter time windows -- 21.0\% cascades have relative potential reach below 0.25 and 33.7\% cascades above 0.75 within 10 minutes span -- comparing to the observation over 14 days (5.1\% and 11.3\%, respectively).

% \header{Impacts on current diffusion model.}
% Root tweet + retweets for constructing a retweet cascade.

% ====================================================


==> Measuring Sampling Effects in Twitter Streaming API/sec-conclusion.tex <==
%!TEX root = TwitterSampling.tex

% ====================================================
\section{Conclusion}
\label{sec:conclusion}

% In this paper, we measure the effects of data sampling when collecting Twitter streaming data.
This work presents a set of in-depth measurements on the effects of Twitter data sampling.
We validate that Twitter rate limit messages closely approximate the volume of missing tweets.
Across different timescales (hour, minute, second, millisecond), we find that the sampling rates have distinct temporal variations at each scale.
We show the effects of sampling across different subjects (entities, networks, cascades), which may in turn distort the results and interpretations of measurement and modeling studies.
For counting statistics such as number of tweets per user and per hashtag, we find that the Bernoulli process with a uniform rate is a reasonable approximation for Twitter data sampling.
We also show how to estimate ground-truth statistics in the complete data by using only the sample data.

\header{Limitations.}
These observations in this paper apply to current Twitter APIs (as of 2020-03) and are subject to the changes of Twitter's proprietary sampling mechanisms.
We are aware of that Twitter plans to release a new set of APIs in near future.
Consistent with the current streaming APIs, the rate limit threshold for the new APIs is also set to 50 tweets per second~\cite{twitterrate2}.
Therefore, we believe the observations of this paper will hold.

\header{Practical implications and future work.}
This work calls attention to the hidden biases in social media data.
We have shown effective methods for estimating ground-truth statistics, which allows researchers to mitigate the risks in their datasets without collecting the complete data.
Our research also provides methods and toolkits for collecting sampled and complete data streams on Twitter.
Our findings provide foundations to many other research topics using sampled data, such as community detection and information diffusion algorithms that are robust to data subsampling.
Future works include measuring a larger set of activity and network measurements under data sampling, generalizing the results of this work to other social media platforms and data formats, and quantifying the robustness of existing network and diffusion models against data sampling. 
% ====================================================


==> Measuring Sampling Effects in Twitter Streaming API/sec-data.tex <==
%!TEX root = TwitterSampling.tex

\input{images/fig-validate-ratemsg.tex}

% ====================================================
\section{Datasets and Twitter rate limit messages}
\label{sec:data}

We collect two datasets, using two sets of keywords employed in recent large-scale studies that use Twitter.
We choose these works because they are high volume and informative for important social science problems (cyberbullying and online content sharing).
We use $\rho$ to denote the sampling rate -- i.e., the probability that a tweet is present in the collected (sampled) dataset.
We use subscripts to differentiate sampling rates that vary over time $\rho_t$, users $\rho_u$, networks $\rho_n$, and cascades $\rho_c$.
The datasets are collected using the Twitter filtered streaming API and are summarized in \Cref{table:dataset}.

\begin{itemize}[leftmargin=*]
  \item \cb~\cite{nand2016bullying}: This dataset tracks all tweets that mention any of the 25 recommended keywords from psychology literature (e.g., \texttt{gay}, \texttt{slut}, \texttt{loser}). The collection period is from 2019-10-13 to 2019-10-26.
  \item \yt~\cite{rizoiu2017expecting}: This dataset tracks all tweets that contain at least one YouTube video URL by using the rule ``\texttt{youtube}'' \texttt{OR} (``\texttt{youtu}'' \texttt{AND} ``\texttt{be}''). The collection period is from 2019-11-06 to 2019-11-19.
\end{itemize}

The streaming client is a program that receives streaming data via Twitter API.
The client will be rate limited if the number of matching tweets exceeds a preset threshold -- 50 tweets per second as of 2020-03~\cite{twitterrate2}.
When we use only one client to track all keywords, we find that both datasets trigger rate limiting.
We refer to the crawling results from a single client as the \textit{sample set}.

We develop a software package ``Twitter-intact-stream''\footnote{\url{https://github.com/avalanchesiqi/twitter-intact-stream}} for constructing the complete data streams on Twitter.
The package splits the filtering predicates into multiple subsets, and tracks each set with a distinct streaming client.
The \cb and \yt datasets are respectively crawled by 8 and 12 clients based on different combinations of keywords and languages.
We remove the duplicate tweets and sort the distinct tweets chronologically.
We refer to the crawling results from multiple clients as the \textit{complete set}.

In very occasional cases, the complete sets also encounter rate limiting.
Estimated from the rate limit messages (detailed next), 0.04\% and 0.14\% tweets in the complete sets are missing, which are negligible comparing to the volumes of missing tweets in the sample sets (47.28\% and 8.47\%, respectively).
For rigorous comparison, we obtain a 30 minutes complete sample from Twitter Firehose and find the difference with our collected data is trivial (detailed in Section C of \cite{appendix}).
Hence, for the rest of this work, we treat the complete sets as if they contain no missing tweets.

%we assume our complete sets are really ``complete''.
% \footnote{The hypothetical maximum volume, i.e., the total volume of collected tweets and estimated missing tweets, should match between the complete set and the sample set. However, in practice they have a small deviation (0.04\% and 0.01\%, respectively) because (1) the streaming API returns duplicate tweets; (2) the streaming clients occasionally disconnect and reconnect to Twitter server.}

\input{tables/tab-data.tex}

% ====================================================

% ====================================================
\header{Validating Twitter rate limit messages.}
When the streaming rate exceeds the threshold, Twitter API emits a rate limit message that consists of a timestamp and an integer.
The integer is designed to indicate the cumulative number of missing tweets since the connection starts~\cite{twitterrate1}.
Therefore, the difference between 2 consecutive rate limit messages should estimate the missing volume in between.

We empirically validate the rate limit messages.
We divide the datasets into a list of segments where (a) they contain no rate limit message in the complete set; (b) they are bounded by 2 rate limit messages in the sample set.
This yields 1,871 and 253 segments in the \cb and \yt datasets, respectively.
The lengths of segments range from a few seconds to several hours, and collectively cover 13.5 days out of the 14-day crawling windows.
In this way, we assure that the segments in the complete set have no tweet missing since no rate limit message is received.
Consequently, for each segment we can compute the volume of missing tweets in the sample set by either computing the difference of the two rate limit messages bordering the segment, or by comparing the collected tweets with the complete set.
\Cref{fig:data-validate-ratemsg}(a) illustrates the collected and missing tweets in an 11-second interval.
The estimated missing volumes from rate limit messages closely match the counts of the missing tweets in the complete set.
Overall, the median error in estimating the missing volume using rate limit messages is less than 0.0005, measured by mean absolute percentage error (MAPE) and shown in \Cref{fig:data-validate-ratemsg}(b).
We thus conclude that the rate limit message is an accurate indicator for the number of missing tweets.
Note that it only approximates the volume of missing tweets, but not the content.

Our observations contradict those from \citet{sampson2015surpassing}, who used the same keyword-splitting approach, yet found that the rate limit messages give inaccurate estimations.
They consistently retrieved more distinct tweets (up to 2 times) than the estimated total volume, i.e., the number of collected tweets plus the estimated missing tweets.
In contrast, our datasets only have a small deviation (0.08\% and 0.13\%, comparing $N_c$ of the complete set to $N_c{+}\hat{N}_m$ of the sample set in \Cref{table:dataset}).
This discrepancy is due to a different implementation choice back in 2015 -- instead of having 1 rate limit message for each second, the rate limit messages were spawned across 4 threads, resulting in up to 4 messages per second.
We provide a detailed analysis in Section C of \cite{appendix}.
% ====================================================


==> Measuring Sampling Effects in Twitter Streaming API/sec-entity.tex <==
%!TEX root = TwitterSampling.tex

% ====================================================
%\section{Measures of entities}
% \section{Sampling and Twitter entity statistics}
\section{Impacts on Twitter entities}
\label{sec:entity}

In this section, we study how the data sampling affects the observed frequency and relative ranking of Twitter entities, e.g., users, hashtags, and URLs.
We first use a Bernoulli process to model the Twitter data sampling (\Cref{ssec:bernoulli}).
Next, we show how the entity statistics for one set (e.g., the complete) can be estimated using the other set (the sample, \Cref{ssec:frequency}).
Finally, we measure the distortions introduced in entity ranking by sampling and how to correct them (\Cref{ssec:ranking}).
The basic statistics of entities are listed in~\Cref{table:entity}.
The analyses in this section, \Cref{sec:network}, and \Cref{sec:cascade}, are done with \cb dataset since its sampling effects are more prominent.

\input{tables/tab-entity.tex}
% ====================================================

% ====================================================
\subsection{Twitter sampling as a Bernoulli process}
\label{ssec:bernoulli}

\input{images/fig-entity-frequency.tex}

We examine how well we can use a Bernoulli process to approximate the Twitter sampling process.
% We propose a model to approximate the Twitter sampling process, and to infer its impact on entity statistics.
Assuming that tweets are sampled identically and independently, the Twitter sampling can be be seen as a simple Bernoulli process with the mean sampling rate $\bar{\rho}$.
% the sampling for each tweet can be seen as a Bernoulli trial with the mean sampling rate $\bar{\rho}$.
% Therefore, the Twitter sampling can be modeled using a simple Bernoulli process with uniform sampling rate $\bar{\rho}$.
We empirically validate this assumption by plotting the complementary cumulative density functions (CCDFs) of user posting frequency (the number of times a user posts) and hashtag frequency (the number of times a hashtag appears) in \Cref{fig:entity-frequency}.
The black and \textcolor{blue}{blue} solid lines respectively show the CCDFs of the complete and the sample sets, while the black dashed line shows the CCDF in a synthetic dataset constructed from the complete set using a Bernoulli process with rate $\bar{\rho}{=}52.72\%$.
% (the mean sampling rate of \cb).
%The distribution of entity frequency is impacted by Twitter sampling.
%% Some entities appear less frequently, some appear the same times, and some disappear entirely.
%\Cref{fig:entity-frequency} shows the complementary cumulative density functions (CCDFs) of user posting frequency (the number of times a user posts) and hashtag frequency (the number of times a hashtag appears).
% the frequency distribution for users and hashtags.
Firstly, we observe that the CCDF of the sample set is shifted left, towards the lower frequency end.
%Moreover, we draw a uniform random sample from the complete set by using the mean sampling rate $\bar{\rho}{=}52.72\%$.
Visually, the distributions for the synthetic (black dashed line) and for the observed sample set (\textcolor{blue}{blue} solid line) overlap each other.
Furthermore, following the practices in~\cite{leskovec2006sampling}, we measure the agreement between these distributions with Kolmogorov-Smirnov D-statistic, which is defined as
%
\begin{equation}
	D(G, G^\prime) = \mathrm{max}_x \{|G(x) - G^\prime(x)|\}
\end{equation}
%
where $G$ and $G^\prime$ are the cumulative distribution functions (CDFs) of two distributions.
With a value between 0 and 1, a smaller D-statistic implies more agreement between two measured distributions.
%We compute the D-statistic between the sample set and the uniform random sample.
The results show high agreement between entity distributions in the synthetic and the observed sample sets (0.0006 for user posting and 0.002 for hashtag).
This suggests that despite the empirical sampling rates not being unique over time, a Bernoulli process of constant rate can model the observed entity frequency distribution well\footnote{We do not choose the goodness of fit test (e.g., Kolmogorov-Smirnov test) because our sample sizes are in the order of millions. And trivial effects can be found to be significant  with very large sample sizes. Instead we report the effect sizes (e.g., D-statistic). Alternative distance metrics (e.g., Bhattacharyya distance or Hellinger distance) yield qualitatively similar results.}.

% \subsection{Estimating complete set statistics}
\subsection{Entity frequency}
\label{ssec:frequency}

We investigate whether the statistics on one set (complete or sample) can be estimated using only the statistics of the other set and the Bernoulli process model.
We use $n_c$ to denote the frequency in the complete set, and $n_s$ the frequency in the sample set ($n_c{\geq}n_s$).
More precisely, we ask these three questions:
What is the distribution of $n_s$ given $n_c{=}k$?
What is the distribution of $n_c$ given $n_s{=}k$?
How many entities are missing altogether given the distribution of $n_s$?
% is greater than or equal to $n_s$.

% Although tweets are not missing at random (see \Cref{sec:random}), we find that 

% Additionally, we ask three questions: (a) given an entity appears $k$ times in the complete set, what is its frequency in the sample set?
% (b) given an entity appears $k$ times in the sample set, what is its frequency in the complete set?
% (c) given the frequency distribution in the sample set, how many entities are entirely missing?
% We define the entity coverage $\gamma$ as the number of entities in the sample set against that in the complete set.

% In the following measurements and inferences, we do not differentiate the temporal sample rates $\rho_t$.
% Instead, we use the mean sampling rate $\bar{\rho}$ for all tweets.
% we make an assumption that all tweets 

%The following measurements and inferences are done on user posting, other entities yield similar results.
%We use $n_c$ to denote the frequency in the complete set and use $n_s$ for the frequency in the sample set.
%$n_c$ is greater than or equal to $n_s$.
%% We aim at quantifying the discrepancies between 
%Assuming the sampling process for each tweet is a Bernoulli trial with a uniform sampling rate $\bar{\rho}$, we quantify how well we can estimate the frequency in one set given the frequency in the other set.

\input{images/fig-entity-binomial.tex}

\header{Modeling sample frequency from the complete set.}

% Now all tweets are with a uniform sampling rate $\bar{\rho}$, the sampling process becomes Bernoulli trials.
% For an entity that appears $n_c$ times, its sample frequency $n_s$ should follow a binomial distribution $B(n_c, \bar{\rho})$.
%Under the independent and identically distributed (i.i.d.) assumption, 
For a user who posts $n_c$ times in the complete set, their sample frequency under the Bernoulli process follows a binomial distribution $B(n_c, \bar{\rho})$.
Specifically, the probability of observing the user $n_s$ times in the sample set is 
%
\begin{equation}
\mathrm{Pr}(n_s | n_c, \bar{\rho}) = {n_c \choose n_s} \bar{\rho}^{n_s} (1{-}\bar{\rho})^{n_c - n_s}
\end{equation}
%
We compute the empirical distribution and binomial distribution for $n_c$ from 1 to 100.
This covers more than 99\% users in our dataset.
\Cref{fig:measure-entity-binomial}(a) shows the D-statistic between two distributions as a function of complete frequency $n_c$.
The binomial distribution models the empirical data better when $n_c$ is smaller.
\Cref{fig:measure-entity-binomial}(b) illustrates an example of $n_c{=}20$.
The binomial distribution closely approximates the empirical distribution.
Their mean sample frequencies (dashed vertical lines) are also identical (10.54).

% 0.24 probability his/her tweets will be observed 5 times, 0.21 probability for 6 times.
% The most likely $n_s$ is 5.

% We adopt the Hellinger distance for measuring the similarity between these two discrete probability distributions.
% The Hellinger distance is defined as the Euclidean norm of the difference of the square root probability,

% \begin{equation}
% \mathrm{H}(A, B) = \frac{1}{\sqrt{2}} ||\sqrt{A} - \sqrt{B}||_2
% \end{equation}

% Hellinger distance is within [0, 1].

\header{Inferring complete frequency from the sample set.}
Under the Bernoulli process, for users who are observed $n_s$ times in the sample set, their complete frequencies follows a negative binomial distribution $NB(n_s, \bar{\rho})$.
The negative binomial distribution models the discrete probability distribution of the number of Bernoulli trials before a predefined number of successes occurs.
In our context, given $n_s$ tweets ($n_s{\geq}1$) are successfully sampled, the probability of having $n_c$ tweets in the complete set is
%
\begin{equation}
\mathrm{Pr}(n_c | n_s, \bar{\rho}) = {n_c{-}1 \choose n_s{-}1} \bar{\rho}^{n_s} (1{-}\bar{\rho})^{n_c - n_s}
\end{equation}
%

\input{images/fig-entity-negbin.tex}

We compute the empirical distribution and negative binomial distribution for $n_s$ from 1 to 100.
\Cref{fig:entity-negbin}(a) shows the D-statistic as a function of sample frequency $n_s$.
Negative binomial distributions models the best when the number of observed tweets is between 9 and 15 (D-statistic${<}$0.02).
\Cref{fig:entity-negbin}(b) shows both distributions for $n_s{=}13$, where the minimal D-statistic is reached.
The negative binomial distribution closely resembles the empirical distribution.
Their estimated mean complete frequencies are very similar (23.60 vs. 23.72, shown as dashed vertical lines).

% The dashed vertical lines map the empirical mean and expected mean of negative binomial distribution. 
% The expected mean of negative binomial distribution is 24.66, computed by $n_s / \rho$.
% This also matches the empirical mean (23.60).
% If we observe a user posting 13 times in the sample set, s/he most likely tweets 22 times ($\mathrm{Pr}{=}0.1$).

\header{Estimating missing volume from the sample set.}
In data collection pipelines, the obtained entities from the filtered stream are sometimes used as seeds for the second step crawling, such as constructing user timelines based on user IDs~\cite{wang2015should}, or querying YouTube statistics based on video URLs~\cite{wu2018beyond}.
However, some entities may be completely missing due to Twitter sampling.
We thus ask: can we estimate the total number of missing entities given the entity frequency distribution of the sample set?
% Although it is expected that most missing entities are with fewer occurrences, we mathematically compute the entity coverage for the whole dataset.

We formulate the problem as solving a matrix equation with constraints.
We use the symbol $\textbf{F}$ to denote the entity frequency vector.
$\textbf{F}[n_s]$ represents the number of entities that occurs $n_s$ times in the sample set.
We want to estimate the frequency vector $\hat{\textbf{F}}$ of the complete set.
For any $n_s$, its sample frequency $\textbf{F}[n_s]$ satisfies
% 
\begin{equation}
\textbf{F}[n_s] = \sum_{k{=}n_s}^{\infty}\mathrm{Pr}(n_s | k, \bar{\rho}) * \hat{\textbf{F}}[k]
\end{equation}
% 
We constrain $\hat{\textbf{F}}$ to be non-negative numbers and decrease monotonically since the frequency distribution is usually heavy-tailed in practice (see~\Cref{fig:entity-frequency}).
We use the frequency vector for $n_s{\in}[1, 100]$.
The above matrix equation can be solved as a constrained optimization task.
For users who post $n_c$ times in the complete set, the probability of their tweets completely missing is $\mathrm{Pr}(n_s{=}0; n_c, \bar{\rho}){=}(1{-}\bar{\rho})^{n_c}$.
Altogether, the estimated missing volume is $\sum_{n_c=1}^{\infty}{(1{-}\bar{\rho})^{n_c} \hat{\textbf{F}}[n_c]}$ for the whole dataset.
We show the estimated results in the rightmost column of \Cref{table:entity}.
The relative errors (MAPE) are smaller than 0.5\% for all entities.
This suggests that the volume of missing entities can be accurately estimated if the frequency distribution of the sample set is observed.

% summary what we show in this section
\header{Summary.}
Although the empirical sample rates have clear temporal variations, we show that we can use the mean sampling rate to estimate some entity statistics, including the frequency distribution and the missing volume.
This reduces the concerns on assuming the observed data stream is a result of uniform random sampling~\cite{joseph2014two,morstatter2014biased,pfeffer2018tampering}.
% Altogether it shows the Twitter sampling is close to uniform random sampling if concerning some collective statistics for the whole dataset.
% ====================================================

% ====================================================
\subsection{Entity ranking}
\label{ssec:ranking}
Entity ranking is important for many social media studies.
One of the most common strategies in data filtering is to keep entities that rank within the top $x$, e.g., most active users or most mentioned hashtags~\cite{morstatter2013sample,gonzalez2014assessing}.
We measure how the Twitter data sampling distorts entity ranking for the most active users, and whether the ground-truth ranking in the complete set can be inferred from the sample ranking.
Note that in this subsection, we allow the sampling rates to be time-dependent $\rho_t$ and user-dependent $\rho_u$ -- as the sampling with a constant rate would preserve the ranking between the complete and the sample sets.
For the universal ranking (considering all entities), we use percentile to measure it and find the higher ranked entities have smaller deviations (detailed in Section E of \cite{appendix}).

% We measure the sampling effects on the ranking of the most active users (in terms of their number of tweets).

% After the sampling, some entities are overrepresented in the sample set, some are underrepresented, and some are entirely missing.

% \header{Finding top entities.}
% The ranking of hashtag in filter stream is a better indicator for the ranking in the complete set (Spearman's rho=0.98), see \cref{fig:measure-case-study}.

% \header{Overrepresented and underrepresented entities.}

% \header{Per entity.}
% Which hashtag/URL will be affected most?
% hashtags and URLs are less distorted as they are collective behaviors from many users.

% \header{Identifying suspicious users.}
\header{Detecting rank distortion.}
\Cref{fig:top-rank}(a) plots the most active 100 users in the sample set on the x-axis, and their ranks in the complete set on the y-axis.
Each circle is colored based on the corresponding user sampling rate $\rho_u$.
The diagonal line indicates uniform random sampling, in which the two sets of ranks should be preserved.
% If the rankings preserve, they should posit along the diagonal line.
The users above the diagonal line improve their ranks in the sample set, while the ones below lose their positions.
\Cref{fig:top-rank}(c) highlights a user \textit{WeltRadio}, who benefits the most from the sampling:
%who gains the most positions among the most active users.
it ranks 50th in the complete set, but it is boosted to 15th place in the sample set.
Comparing the complete tweet volume, its volume (4,529) is only 67\% relative to the user who actually ranks 15th in the complete set (6,728, user \textit{thirdbrainfx}).
We also find that \textit{WeltRadio} tweets mostly in the very high sampling rate secondly period (millisecond 657 to 1,000), resulting in a high user sampling rate ($\rho_u{=}79.1\%$).
On the contrary, \Cref{fig:top-rank}(d) shows a user \textit{bensonbersk} with decreased rank in the sample set and low sampling rate ($\rho_u{=}36.5\%$).
Examining his posting pattern, this user mainly tweets in the low sampling rate hours (UTC-12 to 19).

\input{images/fig-top-rank.tex}

% Which entities appear at higher/lower-than-usual rate, comparing with 100 random samples from the complete set?, see \cref{fig:measure-case-study}.

% \header{Detecting bot-like behaviors from post time.}
% Based on the above observation, we detect the bot-like behaviors from the perspective of user posting time for all users.
% We require the users have at least 100 tweets in the complete set (top 0.5\% active users).
% We use Shannon's entropy

% \begin{equation}
% H(X){=}{-}\sum_{i=1}^{n}P(x_i)log_{b}P(x_i)
% \end{equation}

% to measure the disperse of user posting timestamp.
% As we calculate the probability at each millisecond, we set the base $b$ to 1,000 so that a perfectly even distribution yields to a value of 1.
% Assume a random user has equal probability of posting for each millisecond, i.e., $H(X){=}1$, the smaller $H(X)$ is, the more skewed in the user's posting time distribution, thus more likely such users have scheduled their posting time.

% We examine the score of botness by using an open tool Botometer on the list of top 100 detected users and 100 random users with similar number of post tweets.
% We show the relation between their $H(X)$ with their botness scores.

\header{Estimating true ranking from the sample set.}
Apart from measuring the rank distortion between the complete and the sample sets, we investigate the possibility of estimating the ground-truth ranks by using the observations from the sample set.
From the rate limit messages, we extract the temporal sampling rates that are associated with different timescales (hour, minute, second, and millisecond), i.e., $\rho_t(h,m,s,ms)$.
Based on the negative binomial distribution, for a user who we observe $n_s$ times at timestamp $\kappa{=}(h,m,s,ms)$, the expected volume is $n_s / \rho_t(\kappa)$.
% A valuable question is that if we only observe the sample set, can we correct the entity ranking for better matching the ranks in the complete set?
% We now use the temporal sampling rates which is associated with the posting hour, minute, second, and millisecond.
We compute the estimated tweet volumes for all users and select the most active 100 users.
\Cref{fig:top-rank}(b) shows the estimated ranks on the x-axis and the true ranks on the y-axis.
We quantify the degree of agreement using Kendall's $\tau$, which computes the difference of concordant and discordant pairs between two ranked lists.
With value between 0 and 1, a larger value implies more agreement.
The Kendall's $\tau$ is improved from 0.7349 to 0.8485 with our estimated ranks.
The rank correction is important since it allows researchers to mitigate the rank distortion without constructing a complete data stream.
% ====================================================


==> Measuring Sampling Effects in Twitter Streaming API/sec-intro.tex <==
%!TEX root = TwitterSampling.tex

% ====================================================
\section{Introduction}
\label{sec:intro}

\begin{quote}
\textit{``Polls are just a collection of statistics that reflect what people are thinking in `reality'. And reality has a well-known liberal bias.''}
-- Stephen Colbert\footnote{At the 2006 White House Correspondents' Dinner.} 
% \url{https://en.wikipedia.org/?title=Reality_has_a_well_known_liberal_bias}}
\end{quote}

Data quality is a timely topic that receives broad attention.
The data noises and biases particularly affect data-driven studies in social media~\cite{tufekci2014big,olteanu2019social}.
% One of the main sources of unfairness is data bias, which particularly affects data-driven studies.
Overrepresented or underrepresented data may mislead researchers to spurious claims~\cite{ruths2014social}.
For example, opinion polls wrongly predicted the U.S. presidential election results in 1936 and 1948 because of unrepresentative samples~\cite{mosteller1949pre}.
% \footnote{\url{https://en.wikipedia.org/wiki/Sampling_bias}}.
In the era of machine learning, the data biases can be amplified by the subsequent models.
For example, models overly classify agents doing cooking activity as female due to overrepresented correlations~\cite{zhao2017men}, or lack the capacity to identify dark-skinned women due to underrepresented data~\cite{buolamwini2018gender}.
Hence, researchers must be aware and take account of the hidden biases in their datasets for drawing rigorous scientific conclusions.

Twitter is the most prominent data source in ICWSM -- 82 (31\%) out of 265 full papers in the past 5 years (2015-2019) used Twitter data (listed in Section A of \cite{appendix}),
% \footnote{We list the papers and their used Twitter APIs in Section A of \cite{appendix}.}, 
in part because Twitter has relatively open data policies, and in part because Twitter offers a range of public application programming interfaces (APIs).
Researchers have used Twitter data as a lens to understand political elections~\cite{bovet2019influence}, social movements~\cite{de2016social}, information diffusion~\cite{zhao2015seismic}, and many other social phenomena.
% Twitter delivers a public \textit{filtered} stream by tracking keywords, users, languages, and locations.
Twitter offers two streaming APIs for free, namely \textit{sampled} stream and \textit{filtered} stream.
The filtered stream tracks a set of keywords, users, languages, and locations.
When the matched tweet volume is above a threshold, Twitter subsamples the stream, which compromises the completeness of the collected data.
In this paper, we focus on empirically quantifying the data noises resulted from the sampling in the filtered stream and its impacts on common measurements.

%This defect, which is caused by Twitter APIs, leads to questions such as: How does the data miss? How representative is the sample? Which analyses are impacted? Can the effects be corrected?
This work addresses two open questions related to Twitter data sampling.
Firstly, \textbf{how are the tweets missing in the filtered stream?}
The sampling mechanism of the sampled stream has been extensively investigated~\cite{kergl2014endogenesis,pfeffer2018tampering}, but relatively little is said about the filtered stream.
Since the two streaming APIs are designed to be used in different scenarios, it is pivotal for researchers who use the filtered stream to understand what, when, and how much data is missing.
% Secondly, \textbf{are tweets missing at random?}
% Uniform random sampling yields representative samples, but when the sampling is not uniform, systematic biases may occur.
Secondly, \textbf{what are the sampling effects on common measurements?}
Our work is inspired by~\citet{morstatter2013sample}, who measured the discrepancies of topical, network, and geographic metrics.
We extend the measurements to entity frequency, entity ranking, bipartite graph, retweet network, and retweet cascades.
% Lastly, \textbf{can we correct the sampling effects?}
% A related question is that how large the sample data needs to be for getting the statistics of the complete data~\cite{leskovec2006sampling}.
% Within the scope of Twitter sampling, inferring ground-truth statistics from observed samples remains unexplored.
% Once the above questions are answered, the insights can help 
The answers to these questions not only help researchers shape appropriate questions, but also help platforms improve their data services.

We address the first question by curating two datasets that track suggested keywords in previous studies.
Without leveraging the costly Twitter Firehose service, we construct the complete tweet streams by splitting the keywords and languages into multiple subcrawlers.
We study the Twitter rate limit messages.
Contradicting observations made by \citet{sampson2015surpassing}, our results show that the rate limit messages closely approximate the volume of missing data.
We also find that tweets are not missing at random since the sampling rates have distinct temporal variations across different timescales, especially at the level of hour and millisecond.

Addressing the second question, we measure the effects of Twitter data sampling across different subjects, e.g., the entity frequency, entity ranking, user-hashtag bipartite graph, retweet network, and retweet cascades.
We find that 
(1) the Bernoulli process with a uniform rate can approximate the empirical entity distribution well;
(2) the ranks of top entities are distorted;
(3) the true entity frequency and ranking can be inferred based on sampled observations;
(4) the network structures change significantly with some components more likely to be preserved; 
(5) sampling compromises the quality of diffusion models as the distributions of tweet inter-arrival time and user influence are substantially skewed.
We remark that this work only studies the effects of Twitter sampling mechanism, but does not intend to reverse engineer it.

The main contributions of this work include:
\begin{itemize}[leftmargin=*]
  \item We show that Twitter rate limit message is an accurate indicator for the volume of missing tweets.
  \item A set of measurements on the Twitter data sampling effects across different timescales and different subjects.
  \item We show how to estimate the entity frequency and ranking of the complete data using only the sample data.
  \item We release a software package ``Twitter-intact-stream'' for constructing the complete data streams on Twitter\footnote{The package, collected data, and analysis code are publicly available at \url{https://github.com/avalanchesiqi/twitter-sampling}}.
\end{itemize}

% ====================================================

% \input{tables/tab-notation.tex}

==> Measuring Sampling Effects in Twitter Streaming API/sec-network.tex <==
%!TEX root = TwitterSampling.tex

% ====================================================
\section{Impacts on networks}
% \section{Sampling impacts on networks of entities}
\label{sec:network}

% In this section, we compare the sample set to the complete set.
% We measure the effects of Twitter sampling on entity frequency, entity ranking, bipartite graph, retweet network, and retweet cascade.
% The analyses are done on the \cb dataset as its sampling effects are more prominent.
% though the insights can not directly apply to another dataset, the methods used in this research are applicable.

In this section, we measure the effects of data sampling on two commonly studied networks on Twitter: the user-hashtag bipartite graph, and the user-user retweet network.

% ====================================================

% ====================================================
\subsection{User-hashtag bipartite graph}
\label{ssec:bipartite}

% what are people studying with the bipartite graph?
The bipartite graph maps the affiliation between two disjoint sets of entities.
No two entities within the same set are linked.
Bipartite graphs have been used in many social applications, e.g., mining the relation between scholars and published papers~\cite{newman2001structure}, or between artists and concert venues~\cite{arakelyan2018mining}.
% Notably, the structure of bipartite graph naturally fits the design of collaborative filtering, thus it is also widely used in recommender systems~\cite{konstan2012recommender}.
Here we construct the user-hashtag bipartite graphs for both the complete and the sample sets.
This graph links users to their used hashtags.
Each edge has a weight -- the number of tweets between its associated user and hashtag.
The basic statistics for the bipartite graphs are summarized in \Cref{table:bipartite}.
% All the number reduce, among those, the number of users reduce the most.

% \header{Changes of relative awareness.}
% One can use the hashtag set $\textbf{H}$ as the topical space for representing user interests.
% We define a metric called relative importance $\beta(u, h)$ as the number of tweets with hashtag $h$ from user $u$ -- dubbed $N(u, h)$ -- against the total number of $u$'s tweets,

% \begin{equation}
% \beta(u, h) = N(u, h) / \sum_{h'}^{\textbf{H}}N(u, h')
% \end{equation}

% Here we measure the relative awareness before and after sampling.
% If Twitter sampling is biased towards more active users or more popular hashtags, then their relative awareness will increase.

% \input{images/fig-relative-importance.tex}

% We order the entities by their complete volumes and focus on the most active 1,000 users and most frequently mentioned 1,000 hashtags.
% For each user, we compute the relative importance for all of their hashtags.
% We rank the hashtags by the frequency in the complete set and bin them every 10 percentiles.
% \cref{fig:relative_importance} shows the changes of the relative awareness.
% We can see that the frequent entities become more prominent in the sample set.
% Meanwhile, the less frequent entities lose their relative awareness.
% This suggests that the frequent hashtags for a user will become more frequent in public API feed.
% We find similar trends for the hashtags, users will see the highly active set of users more frequently talk about some hashtags.

% a certain group of users constantly talking about these hashtags.
% If the missing entities are the ones with fewer occurrences, then a public user will see his frequent hashtags more frequently, thus raising the relative awareness.
% The same goes to the hashtags, users will see a certain group of users constantly talking about these hashtags.

% For an active user, are the frequent hashtags more likely to miss or the minority?
% This yields to the relative awareness for this entity.
% We use Shanon's entropy to represent the user dispersiveness of the user interests.
% For hashtags, it represents how they attract attention of general public (general popularity degree).

% \input{images/fig-bipartite-robust.tex}

% \header{Robustness of network measures.}
% Multiple network measures can be applied on the bipartite graph, in this subsection, we investigate which measures are more robust to the Twitter sampling.
% We compute several network measures (e.g., Jaccard, degree centrality, PageRank, and HITS\footnote{For bipartite graph, hubs and authorities scores are interchangeable. All metrics are computed using the \texttt{scikit-network} package.}) in both complete set and sample set.
% We use Kendall's $\tau$ as the measure for discrepancy.
% We focus on the top entities for the rank from 10 to 100.
% From the Jaccard score, the intersection between two lists are much larger than that in the previous study~\cite{morstatter2013sample}.
% We observe that the HITS score is least robust for user, but most robust for hashtag.

% \header{Robustness of network clustering.}
% Perhaps the most common study with bipartite graph is community detection.
%One can project the bipartite graph onto one set of entities, which creates unipartite projection.
%For example, a scientific collaboration network is constructed by linking scholars who have published together~\cite{newman2001structure}.
%We can create a user-user unipartite (based on the common hashtags between users) or a hashtag-hashtag unipartite (based on the common users who use these hashtags).
%A common measurement is to cluster the entities for detecting similar communities.
%To this end, we investigate how the sampling impacts the results of clustering.

\input{tables/tab-bipartite.tex}

\input{images/fig-bipartite-clusters.tex}

\input{tables/tab-clustering.tex}

Clustering techniques are often used to detect communities in such bipartite graphs.
We apply spectral clustering~\cite{stella2003multiclass} on the user-hashtag bipartite graph, with the number of clusters set at 6.
The resulted clusters are summarized in \Cref{table:clustering}, together with the most used 5 hashtags and a manually-assigned category.
Apart from the cyberbullying keywords, there are significant amount of hashtags related to politics, live streaming, and Korean pop culture, which are considered as some of the most discussed topics on Twitter.
We further quantify how the clusters traverse from the complete set to the sample set in \Cref{fig:bipartite-cluster}.
Three of the complete clusters (CC1, CC2, and CC3) are maintained in the sample set (mapping to SC1, SC2, and SC3 respectively), since more than half of the entities preserve.
The remaining three complete clusters disperse.
Investigating the statistics for the complete clusters, the preserved ones have a larger average weighted degree, meaning more tweets between the users and hashtags in these clusters.
Another notable observation is that albeit the entities traverse to the sample clusters differently, all complete clusters have similar missing rates (28\% to 34\%).
It suggests that Twitter data sampling impacts the community structure.
Denser structures are more resilient to sampling.

% ====================================================

% ====================================================
\subsection{User-user retweet network}
\label{ssec:retweet}

\input{images/fig-bowtie.tex}

% add more context if having space
% One can project the bipartite graph onto one set of entities, which creates a unipartite projection.
% For example, a scientific collaboration network is constructed by linking scholars who have published together~\cite{newman2001structure}.
% We can create a user-user unipartite (based on the common hashtags between users) or a hashtag-hashtag unipartite (based on the common users who use these hashtags).
Retweet network describes the information sharing between users.
We build a user-user retweet network by following the ``@RT'' relation..
Each node is a user, and each edge is a directed link weighted by the number of retweets between two users.
The user-user retweet network has been extensively investigated in literature~\cite{sadikov2011correcting,morstatter2013sample,gonzalez2014assessing}.

We choose to characterize the retweet network using the bow-tie structure.
Initially proposed to measure the World Wide Web~\cite{broder2000graph}, the bow-tie structure was also used to measure the QA community~\cite{zhang2007expertise} or YouTube video networks~\cite{wu2019estimating}.
The bow-tie structure characterizes a network into 6 components:
(a) the largest strongly connected component (LSCC) as the central part;
(b) the IN component contains nodes pointing to LSCC but not reachable from LSCC;
(c) the OUT component contains nodes that can be reached by LSCC but not pointing back to LSCC;
(d) the Tubes component connects the IN and OUT components;
(e) the Tendrils component contains nodes pointing from In component or pointing to OUT component;
(f) the Disconnected component includes nodes not in the above 5 components.
\Cref{fig:measure-bowtie} visualizes the bow-tie structure of the user-user retweet network, alongside with the relative size for each component in the complete and sample sets.
The LSCC and IN components, which make up the majority part of the bow-tie, reduce the most in both absolute size and relative ratio due to sampling.
OUT and Tubes are relatively small in both complete and sample sets.
Tendrils and disconnected components enlarge 39\% and 32\% after sampling.

\Cref{fig:measure-bowtie-stats} shows the node flow of each components from the complete set to the sample set.
About a quarter of LSCC component shift to the IN component.
For the OUT, Tubes, Tendrils, and Disconnected components, 20\% to 31\% nodes move into the Tendrils component, resulting in a slight increase of absolute size for Tendrils.
Most notably, nodes in the LSCC has a much smaller chance of missing (2.2\%, other components are with 19\% to 38\% missing rates).
% the LSCC component loses the smallest percentage of nodes due to sampling (2.2\%).
%has a much smaller chance of missing (2.2\%).
% This confirms that the Twitter sampling is biased towards the LSCC component.

% \header{Bow-tie structure of retweet network.}
% bow-tie structure of user following/follower relation \cite{gabielkov2014studying}.

\input{images/fig-bowtie-stats.tex}

% ====================================================


==> Measuring Sampling Effects in Twitter Streaming API/sec-random.tex <==
%!TEX root = TwitterSampling.tex

% ====================================================
\section{Are tweets missing at random?}
\label{sec:random}

% In this section, we validate the method of using the rate limit status to estimate the data loss.
% We also investigate the sampling rate for each tweet.

In this section, we study the randomness of Twitter sampling
%One of the crucial attributes in sampling is the randomness 
-- do all tweets share the same probability of missing?
This is relevant because uniform random sampling creates representative samples.
When the sampling is not uniform, the sampled set may suffer from systematic biases, e.g., some tweets have a higher chance of being observed.
Consequently, some users or hashtags may appear more often than their cohorts.
We tackle the uniformity of the sampling when accounting for the tweet timestamp, language, and type.

\input{images/fig-sampling-rate.tex}

\header{Tweet timestamps.}
% We first examine the sampling rates at different timestamps.
\Cref{fig:temporal-sampling-rates}(a) plots the hourly sampling rates.
\cb dataset has the highest sampling rate ($\rho_t{=}78\%$) at UTC-8.
The lowest sampling rate ($\rho_t{=}41\%$) occurs at UTC-15, about half of the highest value.
\yt dataset is almost complete ($\rho_t{=}100\%$) apart from UTC-8 to UTC-17.
% The lowest sampling rate ($\rho_t{=}76\%$) occurs at UTC-12.
The lowest sampling rate is $76\%$ at UTC-12.
We posit that the hourly variation is related to the overall tweeting dynamics and the rate limit threshold (i.e., 50 tweets per second):
higher tweet volumes yield lower sampling rates.
%, but not fewer tweets in the sample set.
% This is different with~\cite{morstatter2013sample}, in which the authors observed higher tweet volume results in lower sampling rate and fewer tweets.
\Cref{fig:temporal-sampling-rates}(b) shows the sampling rate at the millisecond level, which curiously exhibits a periodicity of one second.
%The most striking observation is sampling rates at the millisecond level, as shown in \Cref{fig:temporal-sampling-rates}(b).
In \cb dataset, the sampling rate peaks at millisecond 657 ($\rho_t{=}100\%$) and drops monotonically till millisecond 550 ($\rho_t{=}6\%$) before bouncing back.
\yt dataset follows a similar trend with the lowest value ($\rho_t{=}76\%$) at millisecond 615.
% \Cref{fig:measure-sampling-rates}(e,f) show that the probability of emitting a tweet is almost the same for every millisecond.
% Therefore, the millisecond variation is related to Twitter's own sampling mechanism.
This artifact leaves the sample set vulnerable to automation tools.
% We observe clear temporal variations of sampling rates in both datasets.
Users can deliberately schedule tweet posting time within the high sampling rate period for inflating their representativeness, or within the low sampling rate period for masking their content in the public API.
% In \Cref{ssec:ranking}, we identify a set of users who may already exploit the sampling artifact.
The minutely and secondly sampling rates are included in Section D of \cite{appendix}.

\input{images/fig-lang-vol.tex}

\input{tables/tab-types.tex}

\header{Tweet languages.}
% The temporal variation motivates us to investigate the sampling rates for different languages.
% Next, we examine the sampling rates for different languages.
% The sampling rates for different languages are also not uniform.
Some languages are mostly used within one particular timezone, e.g., Japanese and Korean\footnote{Japanese Standard Time (JST) and Korean Standard Time (KST) are the same.}.
The temporal tweet volumes for these languages are related to the daily activity patterns in the corresponding countries.
We break down the hourly tweet volumes of \yt dataset into Japanese+Korean and other languages.
The results are shown in \Cref{fig:tweet-lang-vol}.
% English is the most used languages, accounting for 34.2\% tweets.
Altogether, Japanese and Korean account for 31.4\% tweets mentioning YouTube URLs.
The temporal variations are visually different -- 48.3\% of Japanese and Korean tweets are posted in the evening of local time (JST-6pm to 12am), while tweets in other languages disperse more evenly.
Because of the high volume of tweets in this period,  sampling rates within UTC-9 to UTC-15 are lower (see \Cref{fig:temporal-sampling-rates}(a)).
%Because this period has lower sampling rates (see UTC-9 to UTC-15 in 
Consequently, ``ja+ko'' tweets are less likely to be observed (89.0\% in average, 80.9\% between JST-6pm and 12am) than others (92.9\% in average).
%Especially for ``ja+ko'' tweets posted between JST-6pm and 12am, their sampling rate further drops to 80.9\%.

\header{Tweet types.}
Twitter allows the creation of 4 types of tweets.
The users create a \textit{root tweet} when they post new content from their home timelines.
The other 3 types are interactions with existing tweets: \textit{retweets} (when users click on the ``Retweet'' button); \textit{quotes} (when users click on the ``Retweet with comment'' button); \textit{replies} (when users click on the ``Reply'' button).
The relative ratios of different types of tweets are distinct for the two datasets (see \Cref{table:type}).
% are composited differently, as shown in 
% Retweets make up the majority of messages.
\cb has higher ratios of retweets, quotes, and replies than \yt, implying more interactions among users.
However, the ratios of different types are very similar in the sampled versions of both datasets (max deviation$=$0.41\%, retweets in \yt dataset).
%are almost the same before and after sampling 
We conclude that Twitter data sampling is not biased towards any tweet type.

% ====================================================

==> Measuring Sampling Effects in Twitter Streaming API/tables/tab-bipartite.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{table}
    \centering
    \resizebox{.99\columnwidth}{!}{
    \begin{tabular}{rrrr}
        \toprule
         & complete & sample & ratio \\
        \midrule
        \#tweets with hashtags & 24,539,003 & 13,149,980 & 53.59\% \\
        \#users with hashtags & 6,964,076 & 4,758,161 & 68.32\% \\
        avg. hashtags per user & 9.23 & 7.29 & 78.97\% \\
        \#hashtags & 1,166,483 & 880,096 & 75.45\% \\
        avg. users per hashtags & 55.09 & 39.40 & 71.51\% \\
        \bottomrule
    \end{tabular}
    }
    \caption{Statistics of user-hashtag bipartite graph in \cb dataset. Ratio (rightmost column) compares the value of the sample set against that of the complete set, mean sampling rate $\bar{\rho}{=}52.72\%$.}
    \label{table:bipartite}
\end{table}

==> Measuring Sampling Effects in Twitter Streaming API/tables/tab-bowtie.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{table}
    \centering
    \caption{Changes of component size of the bow-tie structure in the complete and the sample set.}
    \label{table:bowtie}
    \resizebox{.95\columnwidthh}{!}{
    \begin{tabular}{rrrrr}
        \toprule
        & \multicolumn{2}{c}{complete} & \multicolumn{2}{c}{sample} \\
        & size & ratio & size & ratio  \\
        \midrule
        LSCC & 1,220,857 & 7.57\% & 672,933 & 5.59\% \\
        IN & 9,622,306 & 59.69\% & 6,152,318 & 51.15\% \\
        OUT & 415,860 & 2.58\% & 317,235& 2.64\% \\
        Tubes & 174,135 & 1.08\% & 168,076 & 1.40\% \\
        Tendrils & 1,991,664 & 12.35\% & 2,066,775 & 17.18\% \\
        Disconnected & 2,696,890 & 16.73\% & 2,650,125 & 22.03\% \\
        Total & 16,121,712 & 100.0\% & 12,027,462 & 100.0\% \\
        \bottomrule
    \end{tabular}
    }
\end{table}


==> Measuring Sampling Effects in Twitter Streaming API/tables/tab-cascade.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{table}
    \centering
    \resizebox{.99\columnwidth}{!}{
    \begin{tabular}{rrrr}
        \toprule
         & complete & sample & ratio \\
        \midrule
        \#cascades & 3,008,572 & 1,168,896 & 38.9\% \\
        \#cascades (${\geq}$50 retweets) & 99,952 & 29,577 & 29.6\% \\
        avg. retweets per cascade & 15.6 & 11.0 & 70.2\% \\
        med. inter-arrival time (s) & 22.9 & 105.7 & 461.6\% \\
        \bottomrule
    \end{tabular}
    }
    \caption{Statistics of cascades in \cb dataset.}
    \label{table:cascade}
\end{table}


==> Measuring Sampling Effects in Twitter Streaming API/tables/tab-clustering.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{table*}
    \centering
    \resizebox{2.09\columnwidth}{!}{
    \begin{tabular}{p{0.3cm}rcccccc}
        \toprule
        \multirow{11}{*}{\rotatebox[origin=c]{90}{complete set}} & & \textbf{CC1} & \textbf{CC2} & \textbf{CC3} & CC4 & CC5 & CC6\\
        & size & \textbf{1,925,520} & \textbf{986,262} & \textbf{742,263} & 1,289,086 & 1,389,829 & 1,562,503  \\
        & \#users & \textbf{1,606,450} & \textbf{939,288} & \textbf{602,845} & 1,080,359 & 1,227,127 & 1,390,276 \\
        & \#hashtags & \textbf{319,070} & \textbf{46,974} & \textbf{139,418} & 208,727 & 162,702 & 172,227 \\
        & avg. degree & \textbf{8.03} & \textbf{7.64} & \textbf{22.19} & 3.46 & 4.74 & 4.07 \\
        & category & \textbf{politics} & \textbf{Korean pop} & \textbf{cyberbullying} & Southeast Asia pop & politics & streaming \\
        \cmidrule{2-8}
        & \multirow{5}{*}{hashtags} & \textbf{brexit} & \textbf{bts} & \textbf{gay} & peckpalitchoke(th) & kamleshtiwari & ps4live \\
        & & \textbf{demdebate} & \textbf{mamavote} & \textbf{pussy} & peckpalitchoke & standwithhongkong & bigolive \\
        & & \textbf{afd} & \textbf{blackpink} & \textbf{sex} & vixx & hongkong & 10tv \\
        & & \textbf{cdnpoli} & \textbf{pcas} & \textbf{horny} & wemadeit & bigil & mixch.tv(ja) \\
        & & \textbf{elxn43} & \textbf{exo} & \textbf{porn} & mayward & lebanon & twitch \\
        \bottomrule
        \toprule
        \multirow{11}{*}{\rotatebox[origin=c]{90}{sample set}} & & \textbf{SC1} & \textbf{SC2} & \textbf{SC3} & SC4 & SC5 & SC6 \\
        & size & \textbf{1,880,247} & \textbf{823,232} & \textbf{551,219} & 822,436 & 549,589 & 805,852 \\
        & \#users & \textbf{1,600,579} & \textbf{767,183} & \textbf{446,303} & 686,609 & 465,339 & 688,922 \\
        & \#hashtags & \textbf{279,668} & \textbf{56,049} & \textbf{104,916} & 135,827 & 84,250 & 116,930 \\
        & avg. degree & \textbf{5.58} & \textbf{5.75} & \textbf{14.98} & 3.06 & 3.51 & 3.28 \\
        & category & \textbf{politics} & \textbf{Korean pop} & \textbf{cyberbullying} & mixed & mixed & mixed \\
        \cmidrule{2-8}
        & \multirow{5}{*}{hashtags} & \textbf{ps4live} & \textbf{bts} & \textbf{gay} & mixch.tv(ja) & bigolive & Idolish7(ja) \\
        & & \textbf{10tv} & \textbf{mamavote} & \textbf{pussy} & bigil & kamleshtiwari & reunion \\
        & & \textbf{brexit} & \textbf{blackpink} & \textbf{sex} & peckpalitchoke(th) & bb13 & Idolish7(ja) \\
        & & \textbf{afd} & \textbf{pcas} & \textbf{horny} & reality\_about\_islam(hi) & biggboss13 & vixx  \\
        & & \textbf{demdebate} & \textbf{bts(ko)} & \textbf{porn} & doki.live(ja) & execution\_rajeh\_mahmoud(ar) & vixx(ko) \\
        \bottomrule
    \end{tabular}
    }
    \caption{Statistics and the most used 5 hashtags in the 6 clusters of the user-hashtag bipartite graph.
    % Clusters are ordered by size (\#users+\#hashtags).
    Three complete clusters maintain their structure in the sample set (\textbf{boldfaced}).
    The language code within brackets is the original language for the hashtag. ja: Japanese; ko: Korean; th: Thai; hi: Hinda; ar: Arabic.}
    \label{table:clustering}
\end{table*}


==> Measuring Sampling Effects in Twitter Streaming API/tables/tab-data.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{table}
    \centering
    \resizebox{.99\columnwidth}{!}{
    \begin{tabular}{rrrrr}
        \toprule
        & \multicolumn{2}{c}{\cb} & \multicolumn{2}{c}{\yt} \\
        & complete & sample & complete & sample \\
        \midrule
        $N_c$ & 114,488,537 & 60,400,257 & 53,557,950 & 49,087,406 \\
        $N_r$ & 3,047 & 1,201,315 & 3,061 & 320,751 \\
        $\hat{N}_m$ & 42,623 & 54,175,503 & 77,055 & 4,542,397 \\
        % $N_c{+}\hat{N}_m$ & 114,531,160 & 114,575,760 & 53,635,005 & 53,629,803 \\
        $\bar{\rho}$ & 99.96\% & 52.72\% & 99.86\% & 91.53\% \\
        \bottomrule
    \end{tabular}
    }
    \caption{Summary of two datasets. $N_c$: \#collected tweets; $N_r$: \#rate limit messages; $\hat{N}_m$: \#estimated missing tweets; $\bar{\rho}$: mean sampling rate. Full specifications for all streaming clients are listed in Section B of \cite{appendix}.}
    \label{table:dataset}
\end{table}

==> Measuring Sampling Effects in Twitter Streaming API/tables/tab-entity.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{table}
    \centering
    \resizebox{.99\columnwidth}{!}{
    \begin{tabular}{rrrrr}
        \toprule
        & complete & sample & \%miss & est. \%miss \\
        \midrule
        \#users & 19,802,506 & 14,649,558 & 26.02\% & 26.12\% \\
        \#hashtags & 1,166,483 & 880,096 & 24.55\% & 24.31\% \\
        \#URLs & 467,941 & 283,729 & 39.37\% & 38.99\% \\
        \bottomrule
    \end{tabular}
    }
    \caption{Statistics of entities in \cb dataset, mean sampling rate $\bar{\rho}{=}52.72\%$.}
    \label{table:entity}
\end{table}

==> Measuring Sampling Effects in Twitter Streaming API/tables/tab-notation.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{table}
    \centering
    \caption{Summary of notations}
    \label{table:notation}
    \begin{tabular}{cp{6cm}}
        \toprule
        Notation & Interpretation\\
        \midrule
        $\rho$ & sampling rate. The probability of presenting in the sample stream.\\
        a & scalars are lowercase \\
        \textbf{x} & vectors are bold lowercase \\
        \textbf{A} & matrices are bold uppercase \\
        $\rho$ & properties in the complete set \\
        $\hat{\rho}$ or $\rho_0$? & hat style, properties in the sample set \\
        \bottomrule
    \end{tabular}
\end{table}

==> Measuring Sampling Effects in Twitter Streaming API/tables/tab-types.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{table}
    \centering
    \resizebox{.99\columnwidth}{!}{
    \begin{tabular}{rrrrr}
        \toprule
        & \multicolumn{2}{c}{\cb} & \multicolumn{2}{c}{\yt} \\
        & complete & sample & complete & sample  \\
        \midrule
        \%root tweets & 14.28\% & 14.26\% & 25.90\% & 26.19\% \\
        \%retweets & 64.40\% & 64.80\% & 62.92\% & 62.51\% \\
        \%quotes & 7.37\% & 7.18\% & 3.44\% & 3.40\% \\
        \%replies & 13.94\% & 13.76\% & 7.74\% & 7.90\% \\
        \bottomrule
    \end{tabular}
    }
    \caption{The ratios of the 4 tweet types (root tweet, retweet, quote, and reply) in the complete and the sample sets.}
    \label{table:type}
\end{table}

==> images/fig-bipartite-robust.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.474\textwidth]{image-files/metrics_kendall.pdf}
	\caption{Kendall's $\tau$ for different network metrics. \textbf{(a)} user; \textbf{(b)} hashtag.}
	\label{fig:bipartite-robust}
\end{figure}

==> images/fig-relative-importance.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.47\textwidth]{image-files/relative_importance.pdf}
	\caption{Changes of relative importance from the complete set to the sample set. \textbf{(a)} user; \textbf{(b)} hashtag.}
	\label{fig:relative_importance}
\end{figure}

==> tables/tab-bowtie.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{table}
    \centering
    \caption{Changes of component size of the bow-tie structure in the complete and the sample set.}
    \label{table:bowtie}
    \resizebox{.95\columnwidthh}{!}{
    \begin{tabular}{rrrrr}
        \toprule
        & \multicolumn{2}{c}{complete} & \multicolumn{2}{c}{sample} \\
        & size & ratio & size & ratio  \\
        \midrule
        LSCC & 1,220,857 & 7.57\% & 672,933 & 5.59\% \\
        IN & 9,622,306 & 59.69\% & 6,152,318 & 51.15\% \\
        OUT & 415,860 & 2.58\% & 317,235& 2.64\% \\
        Tubes & 174,135 & 1.08\% & 168,076 & 1.40\% \\
        Tendrils & 1,991,664 & 12.35\% & 2,066,775 & 17.18\% \\
        Disconnected & 2,696,890 & 16.73\% & 2,650,125 & 22.03\% \\
        Total & 16,121,712 & 100.0\% & 12,027,462 & 100.0\% \\
        \bottomrule
    \end{tabular}
    }
\end{table}


==> tables/tab-notation.tex <==
%!TEX root = ../TwitterSampling.tex

\begin{table}
    \centering
    \caption{Summary of notations}
    \label{table:notation}
    \begin{tabular}{cp{6cm}}
        \toprule
        Notation & Interpretation\\
        \midrule
        $\rho$ & sampling rate. The probability of presenting in the sample stream.\\
        a & scalars are lowercase \\
        \textbf{x} & vectors are bold lowercase \\
        \textbf{A} & matrices are bold uppercase \\
        $\rho$ & properties in the complete set \\
        $\hat{\rho}$ or $\rho_0$? & hat style, properties in the sample set \\
        \bottomrule
    \end{tabular}
\end{table}
